DriCon: On-device Just-in-Time Context Characterization for Unexpected Driving Events

Driving is a complex task carried out under the influence of diverse spatial objects and their temporal interactions. Therefore, a sudden fluctuation in driving behavior can be due to either a lack of driving skill or the effect of various on-road spatial factors such as pedestrian movements, peer vehicles' actions, etc. Therefore, understanding the context behind a degraded driving behavior just-in-time is necessary to ensure on-road safety. In this paper, we develop a system called \ourmethod{} that exploits the information acquired from a dashboard-mounted edge-device to understand the context in terms of micro-events from a diverse set of on-road spatial factors and in-vehicle driving maneuvers taken. \ourmethod{} uses the live in-house testbed and the largest publicly available driving dataset to generate human interpretable explanations against the unexpected driving events. Also, it provides a better insight with an improved similarity of $80$\% over $50$ hours of driving data than the existing driving behavior characterization techniques.

==> sections/Causality_Analysis.tex <==
\section{Feature Study \& Problem Statement}\label{causality-study}
From the previous section, we understand that both driving maneuvers $\mathcal{F}_M$ and various spatial \micro{} $\mathcal{F}_S$ impact driving behavior. However, it is essential to note that \textbf{although all these \micro{} might have a strong correlation with driving behavior, not all of them \textit{cause} poor driving}. Therefore, we first find out the set of \micro{} that \textbf{causes} poor driving, by applying causal inference techniques~\cite{lu2001matching}.

\begin{table*}[!t]
\centering
\caption{Causality Analysis Results}
\label{table:causal}
\scriptsize
\begin{tabular}{|l||l||lllllllllll|}
\hline
                                                                       & \textbf{\begin{tabular}[c]{@{}l@{}}Driving\\ Maneuvers $\mathcal{F}_M$\end{tabular}} & \multicolumn{11}{c|}{\textbf{Spatial \textit{Micro-events} $\mathcal{F}_S$}}                                                                                                                                                                                                                                                                                                                                                                  \\ \hline
\textbf{Initial Set $\mathcal{X}$}                                                   & \textbf{$\mathcal{A}_T$}                                                          & \multicolumn{1}{l|}{\textbf{$\mathcal{O}_T$}}    & \multicolumn{1}{l|}{\textbf{$\mathcal{B}_T$}}    & \multicolumn{1}{l|}{\textbf{$\mathcal{C}_T$}}   & \multicolumn{1}{l|}{\textbf{$\mathcal{P}_T$}}   & \multicolumn{1}{l|}{\textbf{$\mathcal{Q}_T$}}    & \multicolumn{1}{l|}{\textbf{$\mathcal{L}_T$}}    & \multicolumn{1}{l|}{\textbf{$\mathcal{E}_T$}} & \multicolumn{1}{l|}{\textbf{$\mathcal{W}_T$}} & \multicolumn{1}{l|}{\textbf{$\mathcal{G}_T$}} &  \multicolumn{1}{l|}{\textbf{$\mathcal{V}_T$}} & \textbf{$\mathcal{H}_T$}    \\ \hline
\textbf{Tau Co-efficient}    & -0.59                                                                & \multicolumn{1}{l|}{0.696}         & \multicolumn{1}{l|}{-0.54}         & \multicolumn{1}{l|}{-0.57}        & \multicolumn{1}{l|}{-0.56}        & \multicolumn{1}{l|}{-0.74}         & \multicolumn{1}{l|}{-0.61}         & \multicolumn{1}{l|}{-0.31}      & \multicolumn{1}{l|}{-0.52}      & \multicolumn{1}{l|}{-0.53}           & \multicolumn{1}{l|}{0.33}       & -0.6          \\ \hline \hline
\textbf{$\mathcal{ATE}$}                                                           & \textbf{2}                                                           & \multicolumn{1}{l|}{\textbf{1.96}} & \multicolumn{1}{l|}{\textbf{1.92}} & \multicolumn{1}{l|}{\textbf{2.5}} & \multicolumn{1}{l|}{\textbf{0.84}} & \multicolumn{1}{l|}{\textbf{1.7}} & \multicolumn{1}{l|}{\textbf{0.75}} & \multicolumn{1}{l|}{\textcolor{red}{X}}          & \multicolumn{1}{l|}{0.32}       & \multicolumn{1}{l|}{0.48}              & \multicolumn{1}{l|}{\textcolor{red}{X}}        & \textbf{0.92} \\ \hline
\textbf{Treatment Variables $\mathcal{F}$} & $\mathcal{A}_T$                                                                   & \multicolumn{1}{l|}{$\mathcal{O}_T$}             & \multicolumn{1}{l|}{$\mathcal{B}_T$}             & \multicolumn{1}{l|}{$\mathcal{C}_T$}            & \multicolumn{1}{l|}{$\mathcal{P}_T$}            & \multicolumn{1}{l|}{$\mathcal{Q}_T$}             & \multicolumn{1}{l|}{$\mathcal{L}_T$}             & \multicolumn{1}{l|}{--}          &  \multicolumn{1}{l|}{\textcolor{red}{X}}          & \multicolumn{1}{l|}{\textcolor{red}{X}}          & \multicolumn{1}{l|}{--}          & $\mathcal{H}_T$             \\ \hline
\end{tabular}
\end{table*}

%defining the feature set

\subsection{Defining the \textit{Micro-events}}  
The well-established method for causality analysis~\cite{mehrotra2017mytraces} uses three different set of variables -- \textit{treatment variables}, \textit{confounding variables} and \textit{response variable}. Let $\mathcal{F} \subseteq \{\mathcal{F}_M, \mathcal{F}_S\}$ that causes a fluctuation in the driving behavior. We consider $\mathcal{F}$ as the treatment variable and the driving score $\mathcal{R}$ as the response variable against that treatment. To claim that $\mathcal{F}$ influences $\mathcal{R}$, the following two conditions must be satisfied -- (a) $\mathcal{F}$ should always precede $\mathcal{R}$, and (b) there should not be any other variable $\mathcal{Z}$ having a causal impact on $\mathcal{R}$. Here, $\mathcal{Z}$ is known as the confounding variable. Let $\mathcal{X}$ be the set of feature variables corresponding to various \micro{} and driving maneuvers that have a high correlation with $\mathcal{R}$, then $\mathcal{X} = \{\mathcal{F} \cup \mathcal{Z}\}$.  From the existing literature~\cite{yu2016fine} and the pilot study (\S\ref{motiv}), we infer that the feature variables corresponding to the following driving maneuvers $\mathcal{A}_T$ of the ego vehicle at timestamp $T$ of $\mathcal{F}_M$ might impact $\mathcal{R}$ -- Weaving ($\mathcal{A}_T^W$), Swerving ($\mathcal{A}_T^S$), Side-slipping ($\mathcal{A}_T^L$), Abrupt Stop ($\mathcal{A}_T^Q$), Sharp Turns ($\mathcal{A}_T^U$), and Severe Jerkiness ($\mathcal{A}_T^J$). 

Therefore, $\mathcal{A}_T \subseteq \{\mathcal{A}_T^W,  \mathcal{A}_T^S,\mathcal{A}_T^L, \mathcal{A}_T^Q, \mathcal{A}_T^U, \mathcal{A}_T^J \}$.
Similarly, the feature variables corresponding to the following spatial \micro{} from $\mathcal{F}_S$ might impact $\mathcal{R}$. These are $\mathcal{O}_T$ -- Relative Speed ($\mathcal{S}_T$) and Distance ($\mathcal{D}_T$) between the ego and the preceding vehicle ($\mathcal{O}_T \subseteq \{\mathcal{S}_T, \mathcal{D}_T\}$), preceding vehicle's Braking Action ($\mathcal{B}_T$), volume of the peer vehicles in front of the ego vehicle indicating Congestion in the road ($\mathcal{C}_T$), Pedestrian ($\mathcal{P}_T$), Pedestrian's speed ($\mathcal{Q}_T$), Traffic light's color ($\mathcal{L}_T$), Heavy vehicles: \{Bus \& Truck\} ($\mathcal{H}_T$), Light vehicles: \{Bicycle \& Motorcycle\} ($\mathcal{V}_T$), Traffic sign ($\mathcal{E}_T$), Type of  the Road ($\mathcal{G}_T$), and Weather condition ($\mathcal{W}_T$). 

\subsubsection{\textbf{Scoring the Variables}}
We use existing literature~\cite{yolov3, yu2016fine, das2022dribe} to infer $\mathcal{F}_M$ (from inertial features) and $\mathcal{F}_S$ (through video processing) from the BDD dataset. The different variables are scored as follows. We give four different scores to $\mathcal{O}_T$: $0$ -- both $\mathcal{S}_T$ and $\mathcal{D}_T$ are $0$; $1$ -- $\mathcal{S}_T$ is $0$, but $\mathcal{D}_T$ is $1$; $2$ -- $\mathcal{S}_T$ is $1$, but $\mathcal{D}_T$ is $0$; $3$ -- both $\mathcal{S}_T$ and $\mathcal{D}_T$ are $1$. $\mathcal{C}_T$ has been scored with three levels: $0$ -- no congestion (\#vehicles: \{0-5\}), $1$ -- moderate congestion (\#vehicles: \{6-10\}), and $2$ -- heavy congestion (\#vehicles: $>10$). Pedestrian's speed $\mathcal{Q}_T$ is also scored with three levels\footnote{\url{https://www.healthline.com/health/exercise-fitness/average-walking-speed} (Accessed: \today)}: $0$ -- low speed, ($<1.34$m/s) $1$ -- moderate speed (\{$1.34$ - $1.43$\}m/s), and $2$ -- high speed ($>1.43$m/s). Traffic light's color $\mathcal{L}_T$ is encoded as $1$ if color is red; $0$ otherwise. Road type ($\mathcal{G}_T$) is encoded as \{0-3\} for parking, residential, city street and highway. Next, weather conditions ($\mathcal{W}_T$) are encoded as \{0-5\} for clear, overcast, cloudy, rainy, snowy, \& foggy. All other variables are assigned binary scores with $0$ as the presence of the feature (\textit{e.g.,} brake given) and $1$ as the absence of the feature (\textit{e.g.,} no braking).

\subsubsection{\textbf{Computing the Correlation}}
Before diving into computation of causal variables, we compute pair-wise correlation between $\mathcal{R}$ and each variable $f \in \mathcal{X}$ using \textit{Kendall's tau coefficient}. This is to ensure that only the highly correlated features are forwarded to the causal inference computation, as low correlation for a feature is anyway not eligible for being a causal factor. The feature-wise computed correlation values are shown in Table~\ref{table:causal}; traffic sign ($\mathcal{E}_T$) and light vehicle ($\mathcal{V}_T$) exhibit low correlation ($<\abs*{0.5}$), thus get eliminated from $\mathcal{X}$. Detail analysis of the data shows that light vehicles and traffic signs do not adversely affect driving behavior as dedicated lanes are used and signs are well-seen in advance.

\subsubsection{\textbf{Extracting Causal Features}}
Now, we extract the causal features using the filtered variables in $\mathcal{X}$. According to~\cite{rubin1974estimating}, a causal relationship among the treatment ``$\mathcal{F}$'' and response ``$\mathcal{R}$'' variable will exist, if a small change in $\mathcal{F}$ will significantly impact $\mathcal{R}$. This expected change is defined as the \textit{Average Treatment Effect} ($\mathcal{ATE}$). To compute $\mathcal{ATE}$, we need two events, (i) first the treatment is present, (ii) secondly, the treatment is absent. These two events are defined as matching pairs $\mathcal{N}$ to make the observation bias-free~\cite{rubin1974estimating}. For this purpose, we take two drivers $i$ and $j$ with similar trip information; for $i$ treatment is present - $\mathcal{F}(i)$, while for $j$ treatment is absent - $\mathcal{F}(j)$ to generate the matching pairs $\mathcal{N}$. Finally, the $\mathcal{ATE}$ is computed as follows,
\begin{equation}
  \mathcal{ATE} = \mathbb{E}\left(\frac{\mathcal{R}(i)-\mathcal{R}(j)}{\mathcal{X}(i)-\mathcal{X}(j)}\right),\forall(i,j)\in \mathcal{N}
\end{equation}
where, $\mathbb{E}(.)$ is the expectation, $i$ and $j$ are matching pairs and $\mathcal{X}$ = $\mathcal{F} \cup \mathcal{Z}$. The high value of $\mathcal{ATE}$ implies each feature $\in$ $\mathcal{X}$ impacts the driving behavior $\mathcal{R}$ severely. 

\subsection{Lessons Learnt}
The average treatment effects ($\mathcal{ATE}$) for the set of variables $\mathcal{X}$ are shown in Table~\ref{table:causal}. An $\mathcal{ATE}$ value of more than $0.5$ implies a causal relationship between the treatment and the response variable. Clearly, both $\mathcal{F}_M$ and $\mathcal{F}_S$ with their combined features, exhibit a significant high causal impact on $\mathcal{R}$. For individual feature variables, low $\mathcal{ATE}$ values of $\mathcal{G}_T$ and $\mathcal{W}_T$ do not reflect their causal impact over $\mathcal{R}$. As the type of the road and the weather type affect both the treatment variable (say, sharp turn) and the response variable (say, driving behavior), thus a direct causal inference between them is not observed. However, this analysis further makes them eligible for being the confounding variables as $\mathcal{F}_C = \{\mathcal{G}_T \cup \mathcal{W}_T\}$. Therefore, we populate $\mathcal{F}_M = \{\mathcal{A}_T\}$ and $\mathcal{F}_S = \{\mathcal{O}_T \cup \mathcal{B}_T \cup \mathcal{C}_T \cup \mathcal{P}_T \cup \mathcal{Q}_T \cup \mathcal{L}_T \cup \mathcal{H}_T\}$, where $\mathcal{F} \subseteq \{\mathcal{F}_M \bigcup \mathcal{F}_S\}$, impacting driving behavior directly. This causal analysis gives this interesting insight which helps us precisely define the problem statement as follows.

%It is interesting to note that the driving behavior varies across different times of the day (as we observed in Section~\ref{motiv}), particularly because various surrounding factors like road congestion, pedestrian density, movement patterns of the heavy vehicles, etc. change. However, the causal analysis shows that the time of the day does not directly cause poor driving, although it has a good correlation with driving behavior. The same applies to the weather condition that overall impacts the driving situation but is not a causal factor by itself. Instead, these are confounding factors that collectively impact the driving environment (like speed profile of the vehicles, road congestion, pedestrian density, etc.), which in turn works as the causal factors behind poor driving. 
% \highlightsc{It is interesting to note that the driving behavior varies across different times of the day (as we observed in Section~\ref{motiv}), particularly because various surrounding factors like road congestion, pedestrian density, movement patterns of the heavy vehicles, etc. change. However, the causal analysis shows that the time of the day does not directly cause poor driving, although it has a good correlation with driving behavior. The same applies to the weather condition that overall impacts the driving situation but is not a causal factor by itself. Instead, these are confounding factors that collectively impact the driving environment (like speed profile of the vehicles, road congestion, pedestrian density, etc.), which in turn works as the causal factors behind poor driving. The causal analysis gives this interesting insight which helps us precisely define the problem statement as follows.}


\subsection{Problem Statement}
Thus, we define the problem formally as follows. Let $\mathcal{F}^i$ be the set of temporally-represented feature variables corresponding to the driving maneuvers taken and various on-road spatial \micro{} encountered during a trip $i$. Let $\mathcal{R}_T^i$ be the instant driving score at time $T$ during the trip $i$. We are interested in inspecting the events occurred, representing the feature values $\mathcal{F}^i$, when $\abs{\mathcal{R}_T^i - \hat{\mathcal{R}}_{T-1}^i} > \epsilon$ ($\epsilon$ is a hyper-parameter, we set $\epsilon = 1$). Here, $\hat{\mathcal{R}}_{T-1}^i = \ceil{\text{mean}([\mathcal{R}_{1}^i, \mathcal{R}_{T-1}^i])}$. The output of the system is a characterization of \{$\mathcal{F}_M^i$, $\mathcal{F}_S^i$, $\mathcal{F}_C^i$\}, as to whether a fluctuation in the driving behavior is due to the driving maneuvers only ($\mathcal{F}_M^i$) or under the spatially confounding impacted scenario ($\mathcal{F}_S^i$, $\mathcal{F}_C^i$). Finally, we target to generate the explanations based on $\mathcal{F}_M^i$, $\mathcal{F}_S^i$, and $\mathcal{F}_C^i$ to give feedback to the stakeholders for further analysis of the driving profile. Next, we broadly introduce our system architecture.


==> sections/Dataset.tex <==
%\section{Dataset and Motivation}\label{dataset}
%To develop and evaluate the model, we need to extract various driving features for both the target vehicle and its surrounding factors. For this purpose, we rely on a publicly available driving dataset. We primarily use the IMU, GPS, and video data captured through the rear camera (facing towards the front windscreen) of a smartphone mounted on the vehicle's dashboard. 
%The video data serves three purposes. (1) It captures the objects in front of the target vehicle. (2) The video data also provides additional information about the driving environment, like road congestion, factors like weather conditions, etc. (3) Finally, the video data helps us collect the ground truth to validate our proposed model. Additionally, we use the GPS and accelerometer data from the smartphone, which help us extract driving maneuvers taken by the target vehicle. The detail follows.
%\subsection{Dataset and Annotation Drive}\label{bdd}
%We leverage on the largest open-source driving dataset named Berkeley Deep Drive dataset (BDD)~\cite{yu2018bdd100k}, which contains $100$k trips crowd-sourced by $10$k voluntary drivers. The dataset covers $18$ cities across two nations USA and Israel. Each trip comprises $40$ seconds video sequence captured through Nexar\footnote{\url{https://www.getnexar.com/} (Accessed: \today)} devices and driving trajectory information using IMU and GPS sensor data. 
%%The video sequences are of high resolution, i.e., $720$p and $30$ fps frame rate. 
%The smartphone camera captures the front view of the road at $4$ at different times of the day (day, night, dawn, and dusk), $6$ weather conditions (clear, overcast, snowy, rainy, cloudy \& foggy), and $6$ road types (city street, tunnel, highway, residential, parking \& gas station).
\section{Appendix: Annotation Drive on BDD100K Dataset}\label{annotation}
Although the BDD dataset is information-enriched, it does not have annotation labels of how the driver has driven over a trip. Thus, to annotate the driving behavior, we launched an annotation drive. Notably, we quantify the driving behavior with a numeric score on the Likert scale of [1-5], where $1$ denotes the worst driving, and $5$ denotes the best driving. For this purpose, we designed a virtual reality (VR) platform using a web app\footnote{\url{https://drivingskillsvalidator.web.app/} (Accessed: \today)} where the annotators are shown a $40$ seconds driving video clip. Along with that, they are prompted at every $5$ second to rate the driving score on a scale of [1-5] (1 -- Worst driving, 5 -- Best driving) asking, ``\textit{How was the driver driving in the last $5$ seconds?}''. While launching the drive, we also ensure that the annotators use their visual perception using existing driving knowledge and are free from any apriori knowledge about our proposed system, which may induce any bias during the annotation. In this drive, $46$ annotators participated independently, and from the demographic details, we infer the majority of them have driving experience of at least $5$ years. Finally, we annotated $3,800$ trips, where at least $3$ annotators annotated each trip. 

Notably, despite ensuring the bias-free annotation drive, avoiding subjective bias entirely is impossible, as human perception varies subject-wise. For instance, some of the annotators might feel the driving behavior is slightly better than what others think. But it is unlikely that there would be a significant difference between the ratings the three annotators gave. Thus, we calculate the standard deviation among all the annotated scores from that trip to infer the agreement among annotators. We leverage the CDF (see Fig. \ref{fig:pilot-study1})  over the percentage of trips concerning the standard deviation of the annotated driving scores from different annotators. We can observe from Fig. \ref{fig:pilot-study1} that although the standard deviation is not reaching out beyond $1.0$ for $80$\% of the trips, still $20$\% of the trips received random annotations (CDF w/ bias). For the rest of $20$\%, we relaunched the drive, and finally, all the trips have valid annotations (CDF w/o bias). Let $\mathcal{R}^{G}_{T}$ be the mean of all these ground-truth scores from all the annotators at the timestamp $T$. We finally compute $\ceil{\mathcal{R}^{G}_{T}}$, which is called the \textit{instant driving scores}. After the annotation drive, we obtain instant scores ``2'', ``3'', ``4'' \& ``5'' in the ratio of $23$:$23$:$25$:$29$ over all the annotated trips.

\begin{figure}[!t]
    %
    \centering 
    \includegraphics[width=0.7\linewidth,keepaspectratio]{images/cdf_bdd.pdf}
    \caption{Inter-annotator Score Agreement}
    \label{fig:pilot-study1}
\end{figure}



%So, for each trip of length $40$ seconds, we get $8$ instances of driving scores $\ceil{\mathcal{R}^{G}_{T}}$ at an interval of $5$ seconds each. Let $\mathcal{R}^{G}_{T}$ be the mean over all the scoring instances of a single trip, we call $\mathcal{R}^{G}_{T}$ as the \textit{trip score}. Finally, we obtain driving scores ``2'', ``3'', ``4'' \& ``5'' in the ratio of $23$:$23$:$25$:$29$ over all the annotated trips.



==> sections/Feature_Processing.tex <==
\section{Appendix: Feature Processing}\label{feature-process}
We briefly explain the procedure to extract the causal features $\mathcal{F}$ as inferred in \S\ref{problem-statement}.
\subsection{Driving Maneuvers: $\mathcal{F}_M$}
The maneuvers taken by a driver signify their interaction with the road, e.g., (i) while crossing congestion, how often it takes abrupt stops or weaving, (ii) how (s)he handles the poor road conditions (potholes, speed-breaker), etc. We leverage each trip's IMU and GPS data over a $40$ seconds time window. The IMU and GPS data from BDD dataset are already tagged with the smart device's axis (X, Y \& Z), latitude and longitude information. Therefore, we populate the feature vector $\mathcal{A}_T$ at each $5$ second interval $T$ with the following maneuvers adapted from well established methods~\cite{yu2016fine, das2022dribe}: (i) weaving $\mathcal{A}_T^W$, (ii) swerving $\mathcal{A}_T^S$, (iii) side-slipping $\mathcal{A}_T^L$, (iv) abrupt stop $\mathcal{A}_T^O$, (v) sharp turns $\mathcal{A}_T^U$, and (vi) severe jerkiness $\mathcal{A}_T^J$. The detail follows.

\subsubsection{Weaving $\mathcal{A}_T^W$}
We exploit the accelerometer data along the X-axis as this serpentine behavior produces a sinusoidal-like curve deviating from the lateral space to detect weaving. Typically, we characterize weaving signature by observing the curve between the highest and lowest peak of duration $2$ seconds and log the standard deviation along that curve. The sharpness of weaving is signified by the higher magnitude of the standard deviation.  

\subsubsection{Swerving $\mathcal{A}_T^S$}
Next, we detect the swerving signature by observing data along the X and Y-axis of the accelerometer. As swerving is an instantaneous signature, during this maneuver, the peak value rises and falls sharply along the leading and trailing edge of the X-axis. Thus, for a $2$ seconds time window, we observe the highest peak around the curve and inspect that peak further. We log the standard deviation along the leading and trailing edge, which is of $1$ second duration each, around the peak. Along with this, we also validate the condition that the forward movement along the Y-axis remains $\approx 0$. 

\subsubsection{Side-slipping $\mathcal{A}_T^L$}
Similarly, we characterize side-slipping using the X and Y-axis of the accelerometer. The mean and peak value along the X-axis is either positive or negative depending upon the lateral direction (left or right) and rises/falls abruptly from $\approx 0$ within a duration of $2$ second. The standard deviation is also higher during this phase, which is further logged. However, the mean around the Y-axis is slightly $>0$.


\subsubsection{Abrupt Stops $\mathcal{A}_T^O$}
We characterize an abrupt stop using the accelerometer's Y and Z-axis readings. While the ego vehicle is approaching an abrupt stop, the Y-axis value falls to $\approx 0$, and the Z-axis value falls between [0-1], leading to trembles in the vehicle movement.

\subsubsection{Sharp Turns $\mathcal{A}_T^U$}
We identify if the ego vehicle is taking a sharp turn or not by exploiting the GPS data and its latitude and longitude components. Next, we compute the angle of deviation along the GPS-reading trajectory to characterize a turn as the inverse of the tangent angle between the change in latitude and the longitude values. The rise in the magnitude of the angle signifies poor driving.
\subsubsection{Severe Jerkiness $\mathcal{A}_T^J$}
Finally, we identify the jerkiness from the accelerometer data along the X-axis. The first-order derivative of acceleration with respect to the time computes the jerkiness faced throughout the trip. The magnitude of $\mathcal{A}_T^J$ is directly proportionate to the discomfort level of driving.   


\begin{figure}[!ht]
    \centering
    \includegraphics[width=\columnwidth, keepaspectratio]{images/feature.pdf}
    \caption{(a,b) Inferring Pedestrian's Speed, (c) Filtration of Lane Information}
    \label{fig:surr_feature}
\end{figure}
\subsection{Spatial Micro-events: $\mathcal{F}_S$}\label{traffic-obstacles}
To understand the impact of various spatial \micro{} on the driving maneuvers, we leverage the video data over $40$ seconds time window to detect the surrounding causal factors at every $5$ second interval $T$. We describe them next.
\subsubsection{Detected Objects: \{ $\mathcal{P}_T$, $\mathcal{L}_T$ \& $\mathcal{H}_T$ \} }\label{detected-objects}
We use existing video data-based object detection algorithms and further fine-tune them based on our requirements, as developing vision-based algorithms is beyond the scope of our work. For this purpose, we leverage YOLO-V3~\cite{yolov3} algorithm trained on COCO dataset~\cite{lin2014microsoft} to detect a subset of traffic objects such as \textbf{Pedestrians}, \textbf{Cars}, \textbf{Buses}, \textbf{Trucks}, \textbf{Traffic Lights}, \textbf{Bicycles}, and \textbf{Motorcycles}. However, the light vehicles such as \textbf{Bicycles}, and \textbf{Motorcycles} do not impact the driving behavior immediately (\S\ref{problem-statement}), thus we discard them. Next, the remaining objects are chosen to broadly cover the influence of pedestrians' interactions, the presence of heavy vehicles~(buses \& trucks), traffic light signal transitions (red, yellow \& green), and cars on the driving signatures of the driver during the ride, as all the objects detected do not have the similar influence (see \S\ref{motiv}). Moreover, the near-sighted traffic objects around the ego vehicle will impact more than the far-sighted ones. Thus, we further discard the detected objects which depict confidence score $<50\%$ and bounding boxes of area $<10k$, with the intuition that far-sighted objects will have a shorter bounding box area than the near-sighted ones. Another aspect that influences driving behavior is the relative position of traffic objects. The traffic objects in the mid-way of the road, broadly visible from the driver's dashboard, will be of more interest than the left or right lanes, as the ego vehicle will follow them immediately. Thus, we divide each of the frames into $0.2$:$0.6$:$0.2$ ratio along the horizontal axis, as left:middle:right lanes as shown in Fig.~\ref{fig:surr_feature}(c). Therefore, we keep the \textbf{Pedestrians} $\mathcal{P}_T$, \textbf{Cars}, \textbf{Heavy Vehicles} as \{\textbf{Buses} \& \textbf{Trucks}\}  $\mathcal{H}_T$, which have bounding box co-ordinates within the middle lane boundary, and \textbf{Traffic Light Signal Transitions} $\mathcal{L}_T$ without the lane information as traffic lights are often positioned on the left and right lanes. Next, we have already seen from the pilot study that the pedestrians impact the maneuvers taken by a driver more compared to other factors. Consequently, apart from identifying the crossing pedestrians in the mid-way, we also extract their speed next. For running the above pipeline, the video is re-sampled to $15$ frames-per-second, and YOLO-V3 is run on each of the frames. Finally, the mean of each object class count for every $5$ seconds time window is computed.

\subsubsection{Congestion $\mathcal{C}_T$ }
We leverage the mean count of identified cars as described in \S\ref{detected-objects} to derive congestion status as ``low'', ``moderate'', and ``high'' through a user-defined threshold value. Specifically, we denote congestion as low if the count $\in$ [0-5], moderate if it $\in$ [6-10] and high if the value $>10$, respectively.


\subsubsection{Relative Distance $\mathcal{S}_T$ } We extract the relative distance between the ego vehicle and the preceding vehicle using the geometric method of perspective transform~\cite{sun2006road} after identifying the preceding vehicle. This method computes the relative distance by multiplying the geometric distance between the preceding and the ego vehicle by the meters per pixel derived from the resolution of the image frame of the video data.

\subsubsection{Relative Speed $\mathcal{D}_T$}\label{rel_speed} Further, utilizing the relative distance $\mathcal{S}_T$ between the two consecutive frames, we compute the relative speed between the two vehicles. The difference in the relative distance of the two successive frames multiplied by the \textit{fps} represents the relative speed. We implement the pipeline adopted in \cite{udacity}.

\subsubsection{Pedestrian's Speed $\mathcal{Q}_T$ }
A Pedestrian's speed may lead to poor driving behavior, depending on whether (s)he is crossing the road without obeying the traffic guidelines. Thus, we adopt the perspective transformation-based techniques as in ~\S\ref{rel_speed} to infer so. We locate the mid-point along the bottom lateral axis (see Fig. \ref{fig:surr_feature}(a,b)) of the detected pedestrian's bounding box for two consecutive frames. Following this, we compute the difference between ($m_1$ \& $m_2$) that denotes the displacement $m$ with respect to time. Next, the displacement $m$ is converted to meters from pixel using pixel per meter (ppm) derived from image resolution and multiplied with frames per second (fps) of the video to obtain the pedestrian's speed $\mathcal{Q}_T$ in m/s. We encode $\mathcal{Q}_T$ as low, moderate, and high as $<1.34$, $\{1.34-1.43\}$, $>1.43$, respectively, using existing guidelines\footnote{\url{https://www.healthline.com/health/exercise-fitness/average-walking-speed\#average-speed-by-age} (Accessed: \today)}, for further development of the model.   


\subsubsection{Braking Action $\mathcal{B}_T$ }
The preceding vehicle's braking action is signified through the on/off state of the brake lights. For this purpose, we adopt the methodology described in~\cite{das2022dribe}. We use color-transformation techniques such as HSV and grayscale conversion to highlight the brake-lights area of a car. Following this, we train a sequential CNN model to train on the above-mentioned pre-processed images on the KITTI~\cite{kitti} and GTI~\cite{gti} dataset and run this pipeline over our dataset to detect the braking action.

 
